Controllable Context Sensitivity and the Knob Behind It

When making predictions, a language model must trade off how much it relies on its context vs. its prior knowledge. Choosing how sensitive the model is to its context is a fundamental functionality, as it enables the model to excel at tasks like retrieval-augmented generation and question-answering. In this paper, we search for a knob which controls this sensitivity, determining whether language models answer from the context or their prior knowledge. To guide this search, we design a task for controllable context sensitivity. In this task, we first feed the model a context (Paris is in England) and a question (Where is Paris?); we then instruct the model to either use its prior or contextual knowledge and evaluate whether it generates the correct answer for both intents (either France or England). When fine-tuned on this task, instruction-tuned versions of Llama-3.1, Mistral-v0.3, and Gemma-2 can solve it with high accuracy (85-95%). Analyzing these high-performing models, we narrow down which layers may be important to context sensitivity using a novel linear time algorithm. Then, in each model, we identify a 1-D subspace in a single layer that encodes whether the model follows context or prior knowledge. Interestingly, while we identify this subspace in a fine-tuned model, we find that the exact same subspace serves as an effective knob in not only that model but also non-fine-tuned instruct and base models of that model family. Finally, we show a strong correlation between a model's performance and how distinctly it separates context-agreeing from context-ignoring answers in this subspace. These results suggest a single subspace facilitates how the model chooses between context and prior knowledge, hinting at a simple fundamental mechanism that controls this behavior.

==> preamble/bibstyle.tex <==

%\usepackage{natbib}
%\bibliographystyle{abbrvnat}
%\setcitestyle{authoryear,open={(},close={)}} %Citation-related commands

% HYPERREF
\definecolor{darkblue}{RGB}{5, 0, 144}
\usepackage[colorlinks,linktoc=all,breaklinks=true]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=darkblue}
\hypersetup{linkcolor=darkblue}
\hypersetup{urlcolor=darkblue}

% REFERENCING
%\usepackage{inconsolata} % for texttt{}
\usepackage{cleveref}
\crefname{section}{\S}{\S\S}
\Crefname{section}{\S}{\S\S}
\crefname{table}{Tab.}{}
\crefname{figure}{Fig.}{}
\crefname{algorithm}{Algorithm}{}
\crefname{equation}{Eq.}{}
\crefname{appendix}{App.}{}
\crefname{thm}{Theorem}{}
\crefname{prop}{Proposition}{}
\crefname{cor}{Corollary}{}
\crefname{observation}{Observation}{}
\crefname{assumption}{Assumption}{}
\crefformat{section}{\S#2#1#3}

\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother


==> preamble/notation.tex <==

%% MATH
\newcommand{\yijat}{y^{(t)}_{i\xrightarrow{a}j}}
\newcommand{\yat}{y^{(t)}_{a}}
\newcommand{\muijat}{\mu^{(t)}_{i\xrightarrow{a}j}}
\newcommand{\muat}{\mu^{(t)}_{a}}
\newcommand{\lambdaijkt}{\lambda^{(t)}_{i\xrightarrow{k}j}}
\newcommand{\lambdakt}{\lambda^{(t)}_{k}}
\newcommand{\thetatk}{\theta^{(t)}_k}
\newcommand{\rmd}{\mathrm{d}}

\newcommand{\bI}{I}
\newcommand{\bJ}{J}
\newcommand{\bA}{A}
\newcommand{\bT}{T}
\newcommand{\sN}{\boldsymbol{n}}
\newcommand{\sM}{\boldsymbol{m}}


% MATRICES
\def\mY{{\boldsymbol{Y}\xspace}}
\def\mPhi{{\boldsymbol{\Phi}\xspace}}
\def\mPi{{\boldsymbol{\Pi}\xspace}}
\def\mPsi{{\boldsymbol{\Psi}\xspace}}
\def\mLambda{{\boldsymbol{\Lambda}\xspace}}

% METRICS
\newcommand{\PPD}{\textrm{PPD}\xspace}
\newcommand{\MAE}{\textrm{MAE}\xspace}


%% LINK
\newcommand{\link}{github link}





==> preamble/preamble.tex <==
\usepackage{microtype}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{times}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{relsize}
\usepackage{xspace}
\usepackage[hyphens,spaces,obeyspaces]{url}

% Numbers
\usepackage[group-separator={,}]{siunitx}


%% TIKZ
\usepackage{tikz}
\usetikzlibrary{bayesnet}
\usetikzlibrary{arrows}
\usepackage{color}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usetikzlibrary{backgrounds}

%% Table cell colors
\usepackage{hhline}
\usepackage{xcolor}
\usepackage{colortbl}
\definecolor{Grey}{RGB}{210,210,210}



% credits: Tiago Pimentel
%\newcommand{\citeposs}[1]{\citeauthor{#1}'s (\citeyear{#1})}



%%%%%%%%%%%%% MATH
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]

% operators
%% algebraic
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\kron}{\otimes}
\newcommand{\hadamard}{\circ}
\newcommand{\concat}{\circ}
\DeclareMathOperator{\mkvec}{vec}
\newcommand{\detbar}[1]{\left\vert#1\right\vert}
\newcommand{\inv}{^{-1}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\sign}{sign}
%% statistics/stochastic

\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}

% Sets
%% Widely known sets
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\SetSize}[1]{\lvert #1\rvert}

%% sets variables
\def\calA{{\mathcal{A}}}
\def\calB{{\mathcal{B}}}
\def\calC{{\mathcal{C}}}
\def\calD{{\mathcal{D}}}
\def\calE{{\mathcal{E}}}
\def\calF{{\mathcal{F}}}
\def\calG{{\mathcal{G}}}
\def\calH{{\mathcal{H}}}
\def\calI{{\mathcal{I}}}
\def\calJ{{\mathcal{J}}}
\def\calK{{\mathcal{K}}}
\def\calL{{\mathcal{L}}}
\def\calM{{\mathcal{M}}}
\def\calN{{\mathcal{N}}}
\def\calO{{\mathcal{O}}}
\def\calP{{\mathcal{P}}}
\def\calQ{{\mathcal{Q}}}
\def\calR{{\mathcal{R}}}
\def\calS{{\mathcal{S}}}
\def\calT{{\mathcal{T}}}
\def\calU{{\mathcal{U}}}
\def\calV{{\mathcal{V}}}
\def\calW{{\mathcal{W}}}
\def\calX{{\mathcal{X}}}
\def\calY{{\mathcal{Y}}}
\def\calZ{{\mathcal{Z}}}

\def\expect{{\mathbb{E}}}

% Vectors and Matrices both bold-faced
%% Primarily vectors lower cased
\def\vzero{{\mathbf{0}}}
\def\vone{{\mathbf{1}}}
\def\va{{\mathbf{a}}}
\def\vb{{\mathbf{b}}}
\def\vc{{\mathbf{c}}}
\def\vd{{\mathbf{d}}}
\def\ve{{\mathbf{e}}}
\def\vf{{\mathbf{f}}}
\def\vg{{\mathbf{g}}}
\def\vh{{\mathbf{h}}}
\def\vi{{\mathbf{i}}}
\def\vj{{\mathbf{j}}}
\def\vk{{\mathbf{k}}}
\def\vl{{\mathbf{l}}}
\def\vm{{\mathbf{m}}}
\def\vn{{\mathbf{n}}}
\def\vo{{\mathbf{o}}}
\def\vp{{\mathbf{p}}}
\def\vq{{\mathbf{q}}}
\def\vr{{\mathbf{r}}}
\def\vs{{\mathbf{s}}}
\def\vt{{\mathbf{t}}}
\def\vu{{\mathbf{u}}}
\def\vv{{\mathbf{v}}}
\def\vw{{\mathbf{w}}}
\def\vx{{\mathbf{x}}}
\def\vy{{\mathbf{y}}}
\def\vz{{\mathbf{z}}}

% Greek letters
%\def\vtheta{{\boldsymbol{\theta}\xspace}}
\def\veta{{\boldsymbol{\eta}\xspace}}
\def\vmu{{\boldsymbol{\mu}\xspace}}
\def\vsigma{{\boldsymbol{\sigma}\xspace}}
\def\valpha{{\boldsymbol{\alpha}\xspace}}
\def\vdelta{{\boldsymbol{\delta}\xspace}}
\def\vbeta{{\boldsymbol{\beta}\xspace}}
\def\vpi{{\boldsymbol{\pi}\xspace}}
\def\vphi{{\boldsymbol{\phi}\xspace}}
\def\vomega{{\boldsymbol{\omega}\xspace}}
\def\vkappa{{\boldsymbol{\kappa}\xspace}}
\def\vlambda{{\boldsymbol{\lambda}\xspace}}
\def\vtheta{{\boldsymbol{\theta}\xspace}}


%% matrices upper cased
\def\mA{{\mathbf{A}}}
\def\mB{{\mathbf{B}}}
\def\mC{{\mathbf{C}}}
\def\mD{{\mathbf{D}}}
\def\mE{{\mathbf{E}}}
\def\mF{{\mathbf{F}}}
\def\mG{{\mathbf{G}}}
\def\mH{{\mathbf{H}}}
\def\mI{{\mathbf{I}}}
\def\mJ{{\mathbf{J}}}
\def\mK{{\mathbf{K}}}
\def\mL{{\mathbf{L}}}
\def\mM{{\mathbf{M}}}
\def\mN{{\mathbf{N}}}
\def\mO{{\mathbf{O}}}
\def\mP{{\mathbf{P}}}
\def\mQ{{\mathbf{Q}}}
\def\mR{{\mathbf{R}}}
\def\mS{{\mathbf{S}}}
\def\mT{{\mathbf{T}}}
\def\mU{{\mathbf{U}}}
\def\mV{{\mathbf{V}}}
\def\mW{{\mathbf{W}}}
\def\mX{{\mathbf{X}}}
\def\mY{{\mathbf{Y}}}
\def\mZ{{\mathbf{Z}}}

% distributions
\newcommand{\zero}{\mathbf{0}}
\newcommand{\normal}{\mathrm{Normal}}
\newcommand{\gam}{\mathrm{Gamma}}
\newcommand{\zerogeometric}{\mathrm{Zero \text{-} infl. \text{ } Geom.}}
\newcommand{\betabinomial}{\mathrm{BetaBinomial}}
\newcommand{\binomial}{\mathrm{Binomial}}
\newcommand{\betadist}{\mathrm{Beta}}
\newcommand{\categorical}{\mathrm{Categorical}}
\newcommand{\ordered}{\mathrm{Ord}}
\newcommand{\ordnormal}{\mathrm{OrderedNormal}}
\newcommand{\dirichlet}{\mathrm{Dirichlet}}
\newcommand{\poisson}{\mathrm{Poisson}}

% link functions
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}

% macros for common expressions
\newcommand{\half}{\mbox{$\frac{1}{2}$}}
\newcommand{\real}{\mbox{$\mathbb{R}$}}
\newcommand{\indep}{\mbox{$\perp$}}
\newcommand{\ra}{\mbox{$\rightarrow$}}
\newcommand{\lra}{\mbox{$\leftrightarrow$}}
\newcommand{\Ra}{\mbox{$\Rightarrow$}}
\newcommand{\la}{\mbox{$\leftarrow$}}
\newcommand{\indicator}[1]{\mathbbm{1}_{#1}}
\newcommand{\order}[1]{\ensuremath{\mathcal{O}\left(#1\right)}}

% auto-brackets (doesn't work for angle)
\newcommand{\rnd}[1]{\left(#1\right)}
\newcommand{\sqr}[1]{\left[#1\right]}
\newcommand{\crl}[1]{\left\{#1\right\}}

%% CUSTOM_________________________

\newcommand{\defn}[1]{\textit{#1}}
\newcommand{\TechnicalTag}[1]{\texttt{#1}\xspace}
\newcommand{\ttextsc}[1]{\tt{#1}\xspace}
\newcommand{\FOne}{\text{F1}\xspace}
\newcommand{\MSE}{\text{MSE}\xspace}


%% symbols
%\usepackage{tikz}
%\newcommand*\circled[2]{\tikz[baseline=(char.base)]{
%    \node[shape=circle, draw={#2}, inner sep=1pt, scale=0.825, fill=#3] (char) {#1};}}

%% circles
%\newcommand*\Zvar[0]{\circled{Z}{white!20}}
%\newcommand*\eqnsep[0]{\hspace{1cm}}

%% text highlight
%\newcommand*\Zvar[1]{\circled{#1}{blue!20}}


% ALGORITHM CONFIGURATION
\usepackage{algorithm}
\usepackage{algpseudocode}

